Advancing Test-Time Adaptation in Wild Acoustic Test Settings

Acoustic foundation models, fine-tuned for Automatic Speech Recognition (ASR), suffer from performance degradation in wild acoustic test settings when deployed in real-world scenarios. Stabilizing online Test-Time Adaptation (TTA) under these conditions remains an open and unexplored question. Existing wild vision TTA methods often fail to handle speech data effectively due to the unique characteristics of high-entropy speech frames, which are unreliably filtered out even when containing crucial semantic content. Furthermore, unlike static vision data, speech signals follow short-term consistency, requiring specialized adaptation strategies. In this work, we propose a novel wild acoustic TTA method tailored for ASR fine-tuned acoustic foundation models. Our method, Confidence-Enhanced Adaptation, performs frame-level adaptation using a confidence-aware weight scheme to avoid filtering out essential information in high-entropy frames. Additionally, we apply consistency regularization during test-time optimization to leverage the inherent short-term consistency of speech signals. Our experiments on both synthetic and real-world datasets demonstrate that our approach outperforms existing baselines under various wild acoustic test settings, including Gaussian noise, environmental sounds, accent variations, and sung speech.

==> tables/abl_comp.tex <==
% \begin{wraptable}{r}{0cm}
% \centering
% \begin{tabular}{cccccccccccccccccc}
% \toprule[1pt]
%  \multicolumn{6}{c}{Method} & \multicolumn{6}{c}{DSing-dev} & \multicolumn{6}{c}{Dsing-test} \\ \hline 
%  \multicolumn{6}{l}{Ours} & \multicolumn{6}{c}{$53.5$} & \multicolumn{6}{c}{$50.1$}  \\ 
% \multicolumn{6}{l}{w/o TC} & \multicolumn{6}{c}{$54.4$} & \multicolumn{6}{c}{$51.0$}   \\ 
% \multicolumn{6}{l}{w/o ACE} & \multicolumn{6}{c}{$55.7$} & \multicolumn{6}{c}{$54.5$}   \\ 
 
% \bottomrule[1pt]
% \end{tabular}
% \caption{Ablation study of core components on DSing-dev and DSing-test. WER (\%) results are reported.}
% \label{table:abl_comp}
% % \vspace{-5mm}

% \end{wraptable}

\begin{table}
\centering
\begin{minipage}{0.45\textwidth}
\centering
\begin{tabular}{cccccccccccccccccc}
\toprule[1pt]
 \multicolumn{6}{c}{Method} & \multicolumn{6}{c}{DSing-dev} & \multicolumn{6}{c}{DSing-test} \\ 
 % \hline 
 \midrule[0.5pt]
 \multicolumn{6}{l}{Ours} & \multicolumn{6}{c}{$\textbf{53.5}$} & \multicolumn{6}{c}{$\textbf{50.1}$}  \\ 
\multicolumn{6}{l}{w/o STCR} & \multicolumn{6}{c}{$54.4$} & \multicolumn{6}{c}{$51.0$}   \\ 
\multicolumn{6}{l}{w/o CEA} & \multicolumn{6}{c}{$55.7$} & \multicolumn{6}{c}{$54.5$}   \\ 
\bottomrule[1pt]
\end{tabular}
\caption{Ablation study of core components proposed in our work. WER (\%) results are reported.}
\label{subtable:abl_comp}
\end{minipage}%
\hfill
\begin{minipage}{0.45\textwidth}
\centering
\begin{tabular}{cccccccccccccccccc}
\toprule[1pt]
 \multicolumn{6}{c}{Strategy} & \multicolumn{6}{c}{DSing-dev} & \multicolumn{6}{c}{DSing-test} \\ 
 % \hline
 \midrule[0.1pt]
 \multicolumn{6}{l}{Non-Silent} & \multicolumn{6}{c}{$\textbf{53.5}$} & \multicolumn{6}{c}{$\textbf{50.1}$}  \\ 
\multicolumn{6}{l}{Silent} & \multicolumn{6}{c}{$54.9$} & \multicolumn{6}{c}{$51.7$}   \\ 
\multicolumn{6}{l}{All} & \multicolumn{6}{c}{$54.9$} & \multicolumn{6}{c}{$50.6$}   \\ 
\bottomrule[1pt]
\end{tabular}
\caption{Ablation study of strategies for frame selection. WER (\%) results are reported.}
\label{subtable:abl_fil}
\end{minipage}
% \caption{Integrated table with two subtables displayed horizontally}
\end{table}

==> tables/abl_fil.tex <==
\begin{wraptable}{r}{0cm}
\centering
\begin{tabular}{cccccccccccccccccc}
\toprule[1pt]
 \multicolumn{6}{c}{Strategy} & \multicolumn{6}{c}{DSing-dev} & \multicolumn{6}{c}{Dsing-test} \\ \hline 
 \multicolumn{6}{l}{Non-Silent} & \multicolumn{6}{c}{$53.5$} & \multicolumn{6}{c}{$50.1$}  \\ 
\multicolumn{6}{l}{Silent} & \multicolumn{6}{c}{$54.9$} & \multicolumn{6}{c}{$51.7$}   \\ 
\multicolumn{6}{l}{All} & \multicolumn{6}{c}{$54.9$} & \multicolumn{6}{c}{$50.6$}   \\ 
 
\bottomrule[1pt]
\end{tabular}
\caption{Ablation study of selected frames on DSing-dev and DSing-test. WER (\%) results are reported.}
\label{table:abl_fil}
% \vspace{-5mm}

\end{wraptable}

==> tables/accents.tex <==
\begin{table*}[htbp]
\begin{center}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccc}
\toprule[1pt]
 \multicolumn{6}{c}{Method} & \multicolumn{6}{c}{Arabic} & \multicolumn{6}{c}{Mandarin} & \multicolumn{6}{c}{Hindi} & \multicolumn{6}{c}{Korean} & \multicolumn{6}{c}{Spanish} & \multicolumn{6}{c}{Vietnamese} \\ \hline 
 \multicolumn{6}{c}{Source} & \multicolumn{6}{c}{$21.9$} & \multicolumn{6}{c}{$27.5$} & \multicolumn{6}{c}{$17.1$} & \multicolumn{6}{c}{$17.3$} & \multicolumn{6}{c}{$22.2$} & \multicolumn{6}{c}{$34.8$}  \\ 
\multicolumn{6}{c}{Tent} & \multicolumn{6}{c}{$18.9$} & \multicolumn{6}{c}{$23.6$} & \multicolumn{6}{c}{$14.0$} & \multicolumn{6}{c}{$15.0$} & \multicolumn{6}{c}{$19.2$} & \multicolumn{6}{c}{$31.7$}  \\ 
\multicolumn{6}{c}{SAR} & \multicolumn{6}{c}{$20.2$} & \multicolumn{6}{c}{$25.4$} & \multicolumn{6}{c}{$15.3$} & \multicolumn{6}{c}{$16.0$} & \multicolumn{6}{c}{$20.5$} & \multicolumn{6}{c}{$33.4$}  \\ 
\multicolumn{6}{c}{TeCo} & \multicolumn{6}{c}{$18.9$} & \multicolumn{6}{c}{$23.6$} & \multicolumn{6}{c}{$14.0$} & \multicolumn{6}{c}{$15.0$} & \multicolumn{6}{c}{$19.2$} & \multicolumn{6}{c}{$31.7$}  \\ 
 \multicolumn{6}{c}{SUTA}& \multicolumn{6}{c}{$18.2$} & \multicolumn{6}{c}{$22.5$} & \multicolumn{6}{c}{$13.3$} & \multicolumn{6}{c}{$14.3$} & \multicolumn{6}{c}{$18.2$} & \multicolumn{6}{c}{$30.5$}  \\ 
 \multicolumn{6}{c}{Ours} & \multicolumn{6}{c}{$\textbf{18.0}$} & \multicolumn{6}{c}{$\textbf{22.3}$} & \multicolumn{6}{c}{$\textbf{13.2}$} & \multicolumn{6}{c}{$\textbf{14.2}$} & \multicolumn{6}{c}{$\textbf{18.1}$} & \multicolumn{6}{c}{$\textbf{30.4}$}  \\  

% \midrule[1pt]

%  \multicolumn{6}{c}{Unadapted} & \multicolumn{6}{c}{$40.6$} & \multicolumn{6}{c}{$38.8$} & \multicolumn{6}{c}{$43.7$} & \multicolumn{6}{c}{$41.0$}  \\ 
%  \multicolumn{6}{c}{Unadapted w/ LM} & \multicolumn{6}{c}{$41.1$} & \multicolumn{6}{c}{$37.6$} & \multicolumn{6}{c}{$43.5$} & \multicolumn{6}{c}{$40.7$}  \\ 
%  \multicolumn{6}{c}{SUTA} & \multicolumn{6}{c}{$34.9$} & \multicolumn{6}{c}{$33.6$} & \multicolumn{6}{c}{$39.3$} & \multicolumn{6}{c}{$35.9$}  \\ 
%  \multicolumn{6}{c}{SGEM} & \multicolumn{6}{c}{$34.4$} & \multicolumn{6}{c}{$33.0$} & \multicolumn{6}{c}{$38.6$} & \multicolumn{6}{c}{$35.3$}  \\ 
%  \multicolumn{6}{c}{TSTA (Ours)} & \multicolumn{6}{c}{$\textbf{32.9}$} & \multicolumn{6}{c}{$\textbf{30.5}$} & \multicolumn{6}{c}{$\textbf{30.5}$} & \multicolumn{6}{c}{$\textbf{31.3}$}  \\ 



\bottomrule[1pt]
\end{tabular}
\caption{WER (\%) results on L2-Arctic using Wav2vec2 Base with greedy decoding. The best results are bold. }
\label{table:accent}
% \vspace{-5mm}
\end{center}
\end{table*}


==> tables/app_models_large.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{ccccccc}
    \toprule
          & Level 1 & Level 2 & Level 3 & Level 4 & Level 5 & Avg \\
    \midrule
    \multicolumn{1}{l}{Wav2vec2-Large} &       &       &       &       &       &  \\
    \midrule
    Source & 5.0   & 8.1   & 14.6  & 24.9  & 46.9  & 19.9 \\
    Ours  & 4.3   & 6.1   & 9.7   & 15.1  & 31.1  & 13.3 \\
    WERR  & 14.0\% & 24.7\% & 33.6\% & 39.4\% & 33.7\% & 33.2\% \\
    \midrule
    \multicolumn{1}{l}{Hubert-Large} &       &       &       &       &       &  \\
    \midrule
    Source & 5.0   & 6.4   & 8.9   & 12.8  & 24.3  & 11.5 \\
    Ours  & 4.3   & 5.2   & 6.9   & 9.1   & 16.1  & 8.3 \\
    WERR  & 14.0\% & 18.8\% & 22.5\% & 28.9\% & 33.7\% & 27.8\% \\
    \midrule
    \multicolumn{1}{l}{WavLM-Large} &       &       &       &       &       &  \\
    \midrule
    Source & 14.4  & 17.5  & 21.5  & 26.1  & 36.1  & 23.1 \\
    Ours  & 10.7  & 12.4  & 14.5  & 17.1  & 23.9  & 15.7 \\
    WERR  & 25.7\% & 29.1\% & 32.6\% & 34.5\% & 33.8\% & 32.0\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> tables/lm_decode.tex <==
\begin{table*}[htbp]
\begin{center}
\begin{tabular}{cccccc|cccccccccccccccccccccccc}
\toprule[1pt]
\multicolumn{6}{c}{\multirow{2}{*}{Method}} & \multicolumn{6}{c}{\multirow{1}{*}{DSing-dev}} & \multicolumn{6}{c}{\multirow{1}{*}{DSing-test}} & \multicolumn{6}{c}{\multirow{1}{*}{Hansen}}  & \multicolumn{6}{c}{\multirow{1}{*}{Average}} \\  \cline{7-30}
\multicolumn{6}{c}{} & \multicolumn{3}{c}{\multirow{1}{*}{Base}} & \multicolumn{3}{c}{\multirow{1}{*}{Large}} & \multicolumn{3}{c}{\multirow{1}{*}{Base}} & \multicolumn{3}{c}{\multirow{1}{*}{Large}} & \multicolumn{3}{c}{\multirow{1}{*}{Base}} & \multicolumn{3}{c}{\multirow{1}{*}{Large}}  &  \multicolumn{3}{c}{\multirow{1}{*}{Base}} & \multicolumn{3}{c}{\multirow{1}{*}{Large}} \\ \hline

 \multicolumn{6}{c}{Source} & \multicolumn{3}{c}{\multirow{1}{*}{$61.8$}} & \multicolumn{3}{c}{\multirow{1}{*}{$40.6$}} & \multicolumn{3}{c}{\multirow{1}{*}{$60.1$}} & \multicolumn{3}{c}{\multirow{1}{*}{$38.8$}} & \multicolumn{3}{c}{\multirow{1}{*}{$64.3$}} & \multicolumn{3}{c}{\multirow{1}{*}{$43.7$}} & \multicolumn{3}{c}{\multirow{1}{*}{$62.1$}} & \multicolumn{3}{c}{\multirow{1}{*}{$41.0$}}  \\ 
 
 \multicolumn{6}{c}{Source+LM} & \multicolumn{3}{c}{\multirow{1}{*}{$58.6$}} & \multicolumn{3}{c}{\multirow{1}{*}{$41.1$}} & \multicolumn{3}{c}{\multirow{1}{*}{$55.3$}} & \multicolumn{3}{c}{\multirow{1}{*}{$37.6$}} & \multicolumn{3}{c}{\multirow{1}{*}{$60.1$}} & \multicolumn{3}{c}{\multirow{1}{*}{$43.5$}} & \multicolumn{3}{c}{\multirow{1}{*}{$58.0$}} & \multicolumn{3}{c}{\multirow{1}{*}{$40.7$}}  \\ 
 
 \multicolumn{6}{c}{SGEM} & \multicolumn{3}{c}{\multirow{1}{*}{$54.4$}} & \multicolumn{3}{c}{\multirow{1}{*}{$34.4$}} & \multicolumn{3}{c}{\multirow{1}{*}{$50.8$}} & \multicolumn{3}{c}{\multirow{1}{*}{$33.0$}} & \multicolumn{3}{c}{\multirow{1}{*}{$57.8$}} & \multicolumn{3}{c}{\multirow{1}{*}{$38.6$}} & \multicolumn{3}{c}{\multirow{1}{*}{$54.3$}} & \multicolumn{3}{c}{\multirow{1}{*}{$35.3$}}  \\ 

 \multicolumn{6}{c}{Ours} & \multicolumn{3}{c}{\multirow{1}{*}{$\textbf{53.2}$}} & \multicolumn{3}{c}{\multirow{1}{*}{$\textbf{33.3}$}} & \multicolumn{3}{c}{\multirow{1}{*}{$\textbf{50.0}$}} & \multicolumn{3}{c}{\multirow{1}{*}{$\textbf{30.3}$}} & \multicolumn{3}{c}{\multirow{1}{*}{$\textbf{57.7}$}} & \multicolumn{3}{c}{\multirow{1}{*}{$\textbf{37.5}$}} & \multicolumn{3}{c}{\multirow{1}{*}{$\textbf{53.6}$}} & \multicolumn{3}{c}{\multirow{1}{*}{$\textbf{33.7}$}}  \\ 


\bottomrule[1pt]
\end{tabular}
\caption{WER (\%) results on DSing-dev, DSing-test, and Hansen with beam search. Base and Large denote Wav2vec2 Base and Wav2vec2 Large respectively. The best results are bold. }
\label{table:lm_decode}
% \vspace{-5mm}
\end{center}
\end{table*}
